RoboGen: Towards Unleashing Infinite Data for Automated Robot Learning via Generative Simulation

We present RoboGen, a generative robotic agent that automatically learns diverse robotic skills at scale via generative simulation. RoboGen leverages the latest advancements in foundation and generative models. Instead of directly using or adapting these models to produce policies or low-level actions, we advocate for a generative scheme, which uses these models to automatically generate diversified tasks, scenes, and training supervisions, thereby scaling up robotic skill learning with minimal human supervision. Our approach equips a robotic agent with a self-guided propose-generate-learn cycle: the agent first proposes interesting tasks and skills to develop, and then generates corresponding simulation environments by populating pertinent objects and assets with proper spatial configurations. Afterwards, the agent decomposes the proposed high-level task into sub-tasks, selects the optimal learning approach (reinforcement learning, motion planning, or trajectory optimization), generates required training supervision, and then learns policies to acquire the proposed skill. Our work attempts to extract the extensive and versatile knowledge embedded in large-scale models and transfer them to the field of robotics. Our fully generative pipeline can be queried repeatedly, producing an endless stream of skill demonstrations associated with diverse tasks and environments.

==> 3.1_3.2_old.tex <==
\subsection{Task Proposal}
\vspace{-1mm}
\model{} starts with generating meaningful, diverse, and high-level tasks for robots to learn. Instead of directly querying an LLM for task proposal, we initialize the system with a specific robot type and an object randomly sampled from a pool.  The provided robot and sampled object information are then used as input to an LLM to perform task proposal. Such a sampling procedure ensures the diversity of the generated tasks: 
for instance, a legged robot such as a quadruped is capable of acquiring a variety of locomotion skills, while a robotic arm manipulator has the potential to execute a diverse range of manipulation tasks when paired with different sampled objects. This initialization step serves as a seeding stage, providing a basis upon which the LLM can condition and subsequently reason and extrapolate to generate a variety of tasks, taking into account both robot and object affordances. Apart from object-based initialization, another choice is to employ example-based initialization, where we initialize the query with a provided robot and several example tasks sampled from a list 11 pre-defined tasks.

% a legged robot such as a quadruped is suited to learn versatile locomotion skills, and a robotic arm manipulator can perform various kinds of manipulation tasks with different sampled objects.

% Example tasks are "open the door of the storage furniture", "heat a bowl of soup in the oven", and "retrieve the document from the safe". 
% We use the following different methods for generating such common household task descriptions. 

% The first is object-central task proposal, which we use to generate tasks that involve interactions with common household articulated objects.  
We use GPT-4 \citep{gpt4} as the LLM to query in our current pipeline, but this backend can be upgraded once better models are available. In the following,  we explain details of \model{} in the context of a robotic arm (e.g., Franka) and tasks generated pertain to object manipulation, using object-based initialization. In this case, the objects used for initialization are sampled from a predefined list including common articulated and non-articulated objects in household scenarios such as oven, microwave, dispenser, laptop, dishwasher, etc., extracted from PartNetMobility \citep{xiang2020sapien} and RLBench \citep{james2020rlbench}.
% Trained on internet-scale data, LLMs like GPT-4 embeds abundant knowledge on the affordances of these articulated objects, how they can be interacted with, and what tasks they can be used for. 
Having been trained on extensive internet-scale datasets, LLMs like GPT-4 are imbued with a rich understanding of the affordances of these objects, knowledge of how to interact with them, and what kind of meaningful tasks they can be associated with.
% To generate tasks for the robot to interact and manipulate the sampled articulated object, we construct a query to GPT-4 as following. 
In order to generate tasks that involve interaction and manipulation of sampled articulated objects by the robot, we construct a query comprising the broad category to which the articulated object belongs to, its articulation tree derived from the URDF file, and a semantics file providing annotations about the object's links, e.g., which link corresponds to the door in a sampled microwave. This information is provided with the PartNetMobility dataset. 
% The query includes the general category of the articulated object, its articulation tree parsed from the urdf file, and a semantics file that contains annotations of the object's links, e.g., the link is a door in microwave (The urdf and semantics files are shipped with the PartNetMobility dataset). 
The category of the articulated object informs what general types of tasks can be performed with this kind of objects, and the articulation tree and the semantics file informs GPT-4 how exactly the object can be articulated, and semantic meanings of each joint and link. 
The query asks GPT-4 to return a number of tasks that can be performed with the sampled object, where each task consists of the task name, a short description of the task, if there are any other objects that are required for the task besides the provided articulated object, and which joints/links of the articulated object the robot will need to interact with to accomplish the task. Additionally, we include an example input-output pair in the query for GPT-4 to perform in-context learning to improve the quality of its response.

As a concrete example, given a sampled articulated object being a \texttt{microwave}, where \texttt{joint\_0} is a revolute joint connecting its door, and \texttt{joint\_1} being another revolute joint controlling a knob of the timer, GPT-4 would return a task named as ``heat up a bowl of soup'', with a task description of ``The robot arm places a bowl of soup inside the microwave, closes the door and sets the microwave timer for an appropriate heating duration'', additional objects needed for the generated task such as ``A bowl of soup'', and task-relevant joints and links including \texttt{joint\_0} (for opening the microwave door), \texttt{joint\_1} (for setting the timer), \texttt{link\_0} (the door), and \texttt{link\_1} (the timer knob). For the detailed prompt and example responses, please refer to Appendix section B. Note that for cases where we sample non-articulated objects or use example-based initialization, the sampled objects and examples are provided only as a hint for task proposal, and the generated tasks will not be tied to them. For articulated objects, since PartNetMobility is the only articulated object dataset with high quality, and already covers diverse range of articulated assets, we will generate tasks dependent on the sampled asset. For locomotion and soft-body manipulation tasks, we use only example-based initialization, and resort to GPT-4 to populate additional required objects.
By repeatedly querying with different sampled objects and examples, we can generate a diverse range of manipulation and locomotion tasks, concerning the relevant object affordances when needed. 

% The second is example-based task description generation, where we include some examples of common household manipulation tasks in the prompt to GPT-4, and asks it to generate similar tasks. To ensure GPT-4 to generate diverse and different tasks, we randomly sample the tasks used in the prompt from a list of tasks when constructing the prompt. 

% \begin{itemize}
    % \item Object based task generation -- articulated object tasks,
    % \item Tool based task generation -- provide a list of tools.
    % \item Example based task generation -- soft body and rigid object tasks. 
    % \item Group of tasks and their novelties. 
% \end{itemize}

\vspace{-1mm}
\subsection{Scene Generation}
\vspace{-1mm}
Given a proposed task, we proceed to generate a corresponding simulation scene for learning skills to accomplish the task. As shown in Figure~\ref{fig:system}, the scene components and configurations are generated conditioned on the task description, and the object assets are retrieved or generated to populate the simulation scene subsequently.
Specifically, the scene components and configurations are composed of the following elements: queries for relevant assets to be populated into the scene, their physical parameters such as sizes, configurations such as the initial joint angles, and the overall spatial configurations of the assets. 
% As shown in Figure~\ref{fig:system}, the scene configuration includes the their spatial configurations, and physical properties such as sizes. \yufei{align with the figure}.

% The scene components 

% We query GPT-4 to generate all these needed information for building the simulation scene. 
% Specifically, the input to GPT-4 consists of the outputs from the previous step of task proposal, i.e., the name and description of the task, and the objects (and the relevant links and joints) involved in the task.
% For each object involved in the task, we ask GPT-4 to generate the following information for it:
% \begin{itemize}
% We now describe in more detail the information of each asset that needs to be generated for scene configuration.

% \textbf{Asset name}, such that it can be referred to in the simulator.

\textbf{Obtaining queries for relevant assets} Aside from the necessary object assets that are needed for the task generated in the previous step of task proposal, in order to increase the complexity and diversity of the generated scene while resembling object distributions of real-world scenarios, we query GPT-4 to return a number of additional queries for objects that are semantically relevant to the task. See Figure~\ref{fig:teaser} for examples of the additional objects returned by GPT-4 for a task, e.g., for the task ``Open storage, put the toy inside and close it'', the generated scene involves additionally a living room mat, a table-top lamp, a book, and an office chair. 

\textbf{Retrieving or generating assets} The generated queries for relevant objects (i.e. their language descriptions) will be used to either search in an existing database~\citep{deitke2023Objaverse}, or to be used as the input to text-to-image~\citep{midjourney}, and then image-to-3d mesh generation models ~\citep{liu2023zero, poole2022dreamfusion} to generate the 3d textured mesh of the asset.
% \yufei{maybe move this towards the end of this section to align with the figure, }
Specifically, we use Objaverse~\citep{deitke2023Objaverse}, a large-scale dataset containing over 800k object assets (3d meshes, texture pictures, and etc.) as the main database for the retrieval. 
For each object in Objaverse, we obtain a list of language descriptions of it by combining the default annotations and a more cleaned version of annotations from~\citep{luo2023scalable}.  
Given the language description of the asset we want to retrieve, we use Sentence-Bert~\citep{reimers2019sentence} to get the embedding of the description, and retrieve $k$ objects from Objaverse whose language embeddings are the most similar to the language embedding of the target asset. Due to noises in the object annotations, there can be significant discrepancies between the actual asset and the intended target, even when the similarity score in the language embedding space is high. To resolve this, we further leverage a vision-language model (VLM) to verify the retrieved assets and filter out the undesired ones. Specifically, we input an image of the retrieved object to the VLM model, and ask the VLM to caption it. The caption, together with the description of the desired asset and the description of the task, are fed back into GPT-4 to verify if the retrieved asset is appropriate to be used in the proposed task. Since the diverse range of assets from Objaverse is inherently challenging for existing pre-trained models, in order to improve the robustness of our system, we use both Bard \citep{Bard} and BLIP-2 \citep{li2023blip}, to cross verify the validity of the retrieved asset, and adopt the asset only when the captions from both of them are deemed suitable for the task by GPT-4.
% . We tried several vision-language models including instruct Blip, Blip2, mini GPT-4, LLAVA and Bard, and found only Bard is able to accomplish this task reliably with the diverse range of objects from objavarse. 
We use $k=10$ in our pipeline, and if all assets are rejected, we resort to text-to-image followed by image-to-mesh generation models to generate the needed assets from the language description. We use Midjourney~\citep{midjourney} as our text-to-image generative model, and Zero-1-to-3~\citep{liu2023zero} as our image-to-mesh generative model. For soft-body manipulation tasks, in order to obtain a more consistent and controllable target shape for the soft-body under manipulation, we ask GPT-4 to come up with desired target shape, and only use this text-to-image-to-mesh pipeline instead of database retrieval.
% Specifically, we first input the language description to MidJourney~\cite{}, an language to image generation model to generate several candidate images of the object. We then input the image to zero123~\cite{}, an image to mesh model, to generate the texture and mesh of the object. 

\textbf{Asset size} Assets from Objaverse~\citep{deitke2022objaverse} or PartNetMobility~\citep{xiang2020sapien} are usually not of physically plausible sizes. 
To account for this, we query GPT-4 to generate the sizes of the assets such that: 1) the sizes should match real-world object sizes; 2) the relative sizes between objects allow a plausible solution for solving the task, e.g., for the task of ``putting a book into the drawer'', the size of the drawer should be larger than the book. 

\textbf{Initial asset configuration} For certain tasks, the articulated object should be initialized with valid states for the robot to learn the skill. For example, for the task of ``close the window'', the window should be initialized in an open state; similarly, for the task of opening the door, the door should be initially closed. Again, we query GPT-4 to set the initial configurations of these articulated objects, specified in joint angles. To allow GPT-4 to reason about the task and the articulated object, the query script contains the task description, the articulation tree and semantic descriptions of the articulated object.    

\textbf{Scene configuration} 
% specifies the location for each asset in the scene. 
% We make the assumption that the task is either table-top manipulation or not, and GPT-4 will choose between these two cases based on the task description. 
% GPT-4 will decide decide whether the object needs to be placed on a table in common household scenarios, and also its location.  
Scene configuration specifying the location and relevant poses of each asset in the scene is crucial for both producing plausible environments and allowing valid skill learning. E.g., for the task of ``retrieving a document from the safe'', the document needs to be initialized \texttt{inside} the safe; for the task of ``removing the knife from the chopping board'', the knife needs to be initially placed \texttt{on} the chopping board. \model{} queries GPT-4 to generate such special spatial relationships with the task description as the input, and also instructs GPT-4 to place objects in a collision-free manner.

With the generated scene components and configuration, we populate the scene accordingly. See Figure~\ref{fig:teaser} for a collection of example scenes and tasks generated by \model{}.
    
% Among these, we find the most challenging part are 1) find the right object assets to be loaded into the simulator given the language description, and 2) generating the correct spatial configurations of objects needed for the task.

% \begin{itemize}
%     \item objects generation -- 1) search Objaverse and filter by bard; 2) text to image and then to mesh. 
%     \item Spatial configurations.
%     \item Size. 
%     \item Bard verify. 
% \end{itemize}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

